BRIGHTER: BRIdging the Gap in Human-Annotated Textual Emotion Recognition Datasets for 28 Languages

People worldwide use language in subtle and complex ways to express emotions. Although emotion recognition--an umbrella term for several NLP tasks--impacts various applications within NLP and beyond, most work in this area has focused on high-resource languages. This has led to significant disparities in research efforts and proposed solutions, particularly for under-resourced languages, which often lack high-quality annotated datasets. In this paper, we present BRIGHTER--a collection of multi-labeled, emotion-annotated datasets in 28 different languages and across several domains. BRIGHTER primarily covers low-resource languages from Africa, Asia, Eastern Europe, and Latin America, with instances labeled by fluent speakers. We highlight the challenges related to the data collection and annotation processes, and then report experimental results for monolingual and crosslingual multi-label emotion identification, as well as emotion intensity recognition. We analyse the variability in performance across languages and text domains, both with and without the use of LLMs, and show that the BRIGHTER datasets represent a meaningful step towards addressing the gap in text-based emotion recognition.

==> tables/ablation_few_shot.tex <==
\begin{table*}
\centering
\begin{tabular}{lrrrrr}
\toprule
 & Qwen2.5-72B & Dolly-v2-12B & Llama-3.3-70B & Mixtral-8x7B & DeepSeek-R1-70B \\
\midrule
0-shot & 27.03 & 22.46 & 39.66 & 51.11 & 50.42 \\
1-shot & 41.64 & 22.20 & 55.96 & 53.31 & 52.46 \\
2-shot & 32.55 & 35.29 & 59.41 & 55.01 & 52.92 \\
4-shot & 35.87 & 40.13 & 64.95 & 60.06 & 55.55 \\
8-shot & 53.57 & 42.72 & 64.50 & 58.44 & 58.72 \\
16-shot & 66.02 & 41.53 & 65.05 & 61.38 & 59.80 \\
\bottomrule
\end{tabular}
\caption{Ablation on the number of few-shot examples provided to models for the English test set in Track A. Few-shot examples are drawn in equal proportions between positive and negative class from the train set. For an example of few-shot prompts, see \Cref{fig:prompt_example_tracka, fig:prompt_example_trackb} in Appendix ...}
\label{tab:ablation-few-shot}
\end{table*}

==> tables/ablation_prompt_language.tex <==
\begin{table*}
\centering
\begin{tabular}{llrrrr}
\toprule
 &  & Qwen2.5-72B & Dolly-v2-12B & Llama-3.3-70B & Mixtral-8x7B \\
Language & Ablation &  &  &  &  \\
\midrule
\multirow[t]{2}{*}{arq} & Prompt in arq & 43.65 & 23.13 & 24.93 & 48.28 \\
 & Prompt in eng & 29.18 & 40.64 & 49.31 & 49.79 \\
\cline{1-6}
\multirow[t]{2}{*}{chn} & Prompt in chn & 53.36 & 27.16 & 2.48 & 46.21 \\
 & Prompt in eng & 54.71 & 27.66 & 53.94 & 48.22 \\
\cline{1-6}
\multirow[t]{2}{*}{deu} & Prompt in deu & 43.26 & 5.56 & 14.62 & 48.15 \\
 & Prompt in eng & 54.57 & 21.50 & 54.55 & 53.51 \\
\cline{1-6}
\multirow[t]{2}{*}{hau} & Prompt in eng & 41.45 & 30.31 & 47.00 & 39.29 \\
 & Prompt in hau & 41.44 & 26.10 & 10.83 & 17.49 \\
\cline{1-6}
\multirow[t]{2}{*}{hin} & Prompt in hin & 63.54 & 25.90 & 3.36 & 45.34 \\
 & Prompt in eng & 79.41 & 27.81 & 70.29 & 59.54 \\
\cline{1-6}
\multirow[t]{2}{*}{mar} & Prompt in eng & 74.37 & 28.42 & 68.97 & 54.97 \\
 & Prompt in mar & 61.10 & 16.36 & 4.60 & 38.18 \\
\cline{1-6}
\multirow[t]{2}{*}{ptbr} & Prompt in ptbr & 48.68 & 23.57 & 28.83 & 37.80 \\
 & Prompt in eng & 51.66 & 24.02 & 45.29 & 44.17 \\
\cline{1-6}
\multirow[t]{2}{*}{swe} & Prompt in swe & 47.38 & 15.90 & 31.30 & 45.20 \\
 & Prompt in eng & 47.48 & 20.41 & 49.19 & 47.41 \\
\cline{1-6}
\multirow[t]{2}{*}{ukr} & Prompt in eng & 44.45 & 18.22 & 42.20 & 40.52 \\
 & Prompt in ukr & 42.04 & 15.18 & 18.12 & 35.82 \\
\cline{1-6}
\multirow[t]{2}{*}{vmw} & Prompt in vmw & 17.27 & 16.82 & 16.44 & 15.16 \\
 & Prompt in eng & 21.39 & 16.45 & 18.48 & 17.59 \\
\cline{1-6}
\bottomrule
\end{tabular}
\caption{Ablation comparing when prompts are provided in English language against when prompts are provided in the target language for multi-label emotion recognition. For a full list of prompts, refer to \Cref{tab:multilang-prompts} in Appendix ...}
\label{tab:ablation-multilingual-prompts}
\end{table*}

==> tables/ablation_prompt_versions.tex <==
\begin{table*}
\centering
\begin{tabular}{lrrrrr}
\toprule
 & Qwen2.5-72B & Dolly-v2-12B & Llama-3.3-70B & Mixtral-8x7B & DeepSeek-R1-70B \\
\midrule
Prompt v1 & 58.29 & 36.53 & 62.13 & 61.15 & 57.17 \\
Prompt v2 & 57.98 & 42.26 & 66.34 & 59.35 & 59.79 \\
Prompt v3 & 58.95 & 44.51 & 63.17 & 64.64 & 55.09 \\
\bottomrule
\end{tabular}
\caption{Ablation on different paraphrases of the prompt provided to models for the English test set in Track A. $^*$For the full prompts, please refer to \Cref{tab:prompt-variants} in Appendix ...}
\label{tab:ablation-prompt-variants}
\end{table*}

==> tables/ablation_topk.tex <==
\begin{table*}
\centering
\begin{tabular}{lrrrrr}
\toprule
 & Qwen2.5-72B & Dolly-v2-12B & Llama-3.3-70B & Mixtral-8x7B & DeepSeek-R1-70B \\
\midrule
@1 & 54.63 & 41.11 & 66.48 & 57.46 & 58.61 \\
@2 & 65.48 & 51.63 & 74.73 & 68.09 & 72.36 \\
@4 & 67.74 & 65.19 & 79.46 & 69.26 & 84.68 \\
@8 & 73.81 & 70.32 & 82.74 & 71.62 & 91.17 \\
\bottomrule
\end{tabular}
\caption{Ablation on the top$_k$ performance-- meaning whether the gold answer was present in $k$ parallel generations of the language model--for the English test set in Track A.}
\label{tab:ablation-topk}
\end{table*}

==> tables/class_dist.tex <==
\begin{table}[t]
  \small
  \centering
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.1}
  \rowcolors{2}{gray!6}{white}
  \begin{tabular}{@{}lrrrrrrr@{}}
    \toprule
    \textbf{Lan.} & \textbf{Anger} & \textbf{Disgust} & \textbf{Fear} & \textbf{Joy} & \textbf{Sadness} & \textbf{Surprise} & \textbf{Other} \\ 
    \midrule
    \texttt{afr} & 132 & 88 & 252 & 958 & 365 & 0 & 892 \\
    \texttt{arq} & 620 & 436 & 465 & 326 & 849 & 650 & 196 \\
    \texttt{ary} & 636 & 116 & 202 & 504 & 415 & 414 & 757 \\
    \texttt{chn} & 2432 & 852 & 150 & 1103 & 762 & 388 & 1224 \\
    \texttt{deu} & 1605 & 1718 & 506 & 1139 & 1083 & 336 & 603 \\
    \texttt{eng} & 671 & 0 & 3218 & 1375 & 1794 & 1669 & 293 \\
    \texttt{esp} & 929 & 1275 & 549 & 1237 & 586 & 855 & 0 \\
    \texttt{hau} & 684 & 552 & 549 & 535 & 1084 & 583 & 461 \\
    \texttt{hin} & 599 & 386 & 540 & 644 & 635 & 434 & 781 \\
    \texttt{ibo} & 965 & 898 & 366 & 778 & 822 & 128 & 1050 \\
    \texttt{ind} & 209 & 196 & 79 & 495 & 296 & 316 & 65 \\
    \texttt{jav} & 205 & 101 & 113 & 356 & 317 & 363 & 189 \\
    \texttt{kin} & 743 & 208 & 236 & 704 & 1053 & 175 & 1180 \\
    \texttt{mar} & 528 & 408 & 544 & 655 & 655 & 449 & 601 \\
    \texttt{pcm} & 561 & 3144 & 676 & 951 & 1648 & 1643 & 306 \\
    \texttt{ptbr} & 1475 & 151 & 256 & 1198 & 693 & 331 & 1020 \\
    \texttt{ptmz} & 151 & 107 & 182 & 332 & 460 & 167 & 736 \\
    \texttt{ron} & 440 & 600 & 834 & 904 & 755 & 908  & 203 \\
    \texttt{rus} & 816 & 421 & 457 & 782 & 601 & 504 & 766 \\
    \texttt{sun} & 186 & 150 & 103 & 1490 & 471 & 501 & 52 \\
    \texttt{swa} & 520 & 398 & 155 & 740 & 582 & 894 & 1285 \\
    \texttt{swe} & 530 & 479 & 68 & 1043 & 296 & 124 & 722 \\
    \texttt{tat} & 303 & 247 & 123 & 416 & 479 & 272 & 360 \\
    \texttt{ukr} & 209 & 174 & 340 & 821 & 665 & 390 & 1551 \\
    \texttt{vmw} & 151 & 107 & 183 & 332 & 463 & 167 & 736 \\
    \texttt{xho} & 93 & 11 & 44 & 707 & 939 & 363 & 595 \\
    \texttt{yor} & 325 & 135 & 130 & 454 & 1393 & 424 & 2364 \\
    \texttt{zul} & 240 & 84 & 94 & 172 & 601 & 263 & 1182 \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Distribution of emotion classes}. Classes with a value of 0 indicate the absence of the emotional class in the corresponding language in the dataset.}
  \label{tab:class_distribution}
\end{table}



==> tables/data_split.tex <==

\begin{table}[ht]
  \small
 \resizebox{\linewidth}{!}{
  \centering
  %\setlength{\tabcolsep}{4pt}
  %\renewcommand{\arraystretch}{1.1}
  \begin{tabular}{@{}lrrrrrr@{}}
    \toprule
    \textbf{Lang.} & \textbf{Train} & \textbf{Dev} & \textbf{Test} &\textbf{Total} \\ 
    \midrule
    \texttt{afr}  & 2,107 & 98  & 1,065 &\\
    \texttt{arq}  & 901  & 100 & 902  &\\
    \texttt{ary}  & 1,608 & 267 & 812  &\\
    \texttt{chn}  & 2.642 & 200 & 2,642 &\\
    \texttt{deu}  & 2,603 & 200 & 2,604 &\\
    \texttt{eng}  & 2,768 & 116 & 2,767 &\\
    \texttt{esp}  & 1,996 & 184 & 1,695 &\\
    \texttt{hau}  & 2,145 & 356 & 1,080 &\\
    \texttt{hin}  & 2,556 & 100 & 1,010 &\\
    \texttt{ibo}  & 2,880 & 479 & 1,444 &\\
    \texttt{ind}  & --    & 156 & 851  &\\
    \texttt{jav}  & --    & 151 & 837  &\\
    \texttt{kin}  & 2,451 & 407 & 1,231 &\\
    \texttt{mar}  & 2,415 & 100 & 1,000 &\\
    \texttt{pcm}  & 3,728 & 620 & 1,870 &\\
    \texttt{ptbr} & 2,226 & 200 & 2,226 &\\
    \texttt{ptmz} & 1,546 & 257 & 776  &\\
    \texttt{rus}  & 2,679 & 199 & 1,000 &\\
    \texttt{sun}  & 9,24  & 199 & 926  &\\
    \texttt{swa}  & 3,307 & 551 & 1,656 &\\
    \texttt{swe}  & 1,187 & 200 & 1,188 &\\
    \texttt{tat}  & 1,000 & 200 & 1,000 &\\
    \texttt{ukr}  & 2,466 & 249 & 2,234 &\\
    \texttt{vmw}  & 1,551 & 258 & 777  &\\
    \texttt{xho}  & --   & 682 & 1,594 &\\
    \texttt{yor}  & 2,992 & 497 & 1,500 &\\
    \texttt{zul}  & --    & 875 & 2,047 &\\
    \bottomrule
  \end{tabular}
}
  \caption{Sizes of train, dev, test splits and sizes of the different \datasetname datasets. '--' indicates no training data.}
  \label{tab:data_split}
\end{table}






%\begin{table*}[h]
%\resizebox{\textwidth}{!}{
%  \centering
%  \setlength{\tabcolsep}{4pt}
%  \renewcommand{\arraystretch}{1.1}
%  \begin{tabular}{@{}lccccccccccccccccccccccccccc@{}}
%    \toprule
%    & \texttt{afr} & \texttt{arq} & \texttt{ary} & \texttt{chn} & \texttt{deu} & \texttt{eng} & \texttt{esp} & \texttt{hau} & \texttt{hin} & \texttt{ibo} & \texttt{ind} & \texttt{jav} & \texttt{kin} & \texttt{mar} & \texttt{pcm} & \texttt{ptbr} & \texttt{ptmz} & \texttt{rus} & \texttt{sun} & \texttt{swa} & \texttt{swe} & \texttt{tat} & \texttt{ukr} & \texttt{vmw} & \texttt{xho} & \texttt{yor} & \texttt{zul} \\ 
%    \midrule
%    \textbf{Train} & 2,107 & 901 & 1,608 & 2,642 & 2,603 & 2,768 & 1,996 & 2,145 & 2,556 & 2,880 & -- & -- & 2,451 & 2,415 & 3,728 & 2,226 & 1,546 & 2,679 & 924 & 3,307 & 1,187 & 1,000 & 2,466 & 1,551 & -- & 2,992 & -- \\
%    \textbf{Dev} & 98 & 100 & 267 & 200 & 200 & 116 & 184 & 356 & 100 & 479 & 156 & 151 & 407 & 100 & 620 & 200 & 257 & 199 & 199 & 551 & 200 & 200 & 249 & 258 & 682 & 497 & 875 \\
%    \textbf{Test} & 1,065 & 902 & 812 & 2,642 & 2,604 & 2,767 & 1,695 & 1,080 & 1,010 & 1,444 & 851 & 837 & 1,231 & 1,000 & 1,870 & 2,226 & 776 & 1,000 & 926 & 1,656 & 1,188 & 1,000 & 2,234 & 777 & 1,594 & 1,500 & 2,047 \\
%   \bottomrule
%  \end{tabular}
%  }
%  \caption{\textbf{Data split by language.} The table shows the number of examples in the Train, Dev, and Test sets. '--' indicates no training data.}
%  \label{tab:data_split}
%\end{table*}


==> tables/shcmp_english.tex <==
\begin{table}[t]
  \small
    \centering
    \setlength{\tabcolsep}{4pt} 
    \renewcommand{\arraystretch}{1.1} 
    \begin{tabular}{@{}ccccc@{}}
        \toprule
        \textbf{\#Bins} & \textbf{Bin Size} & \textbf{Exp. SHCMP} & \textbf{SHCMP} \\ 
        & & (\%) & (\%) \\ 
        \midrule
        10 & 0.60 & 10.0 & 69.28 \\ 
         7 & 0.86 & 14.3 & 69.15 \\ 
         5 & 1.20 & 20.0 & 81.86 \\ 
         4 & 1.50 & 25.0 & 81.97 \\ 
         3 & 2.00 & 33.3 & 84.28 \\ 
         2 & 3.00 & 50.0 & 90.18 \\ 
        \bottomrule
    \end{tabular}
    \caption{SHCMP (\%) values for English annotations across varying numbers of bins. Larger bin sizes result in higher SHCMP scores, indicating improved reliability for coarser-grained categories.}
    \label{tab:shcmp-english}
\end{table}

==> tables/track_a_llms.tex <==
\begin{table*}
\begin{tabular}{lrrrrr}
\toprule
 & Qwen2.5-72B & Dolly-v2-12B & Llama-3.3-70B & Mixtral-8x7B & DeepSeek-R1-70B \\
\midrule
afr & 60.18 & 23.58 & 61.28 & 53.69 & 43.66 \\
% amh & 37.82 & 5.10 & 42.84 & 29.00 & 36.89 \\
arq & 37.78 & 38.59 & 55.75 & 45.29 & 50.87 \\
ary & 52.76 & 24.27 & 44.96 & 35.07 & 47.21 \\
chn & 55.23 & 27.52 & 53.36 & 44.91 & 53.45 \\
deu & 59.17 & 26.86 & 56.99 & 51.20 & 54.26 \\
eng & 55.72 & 42.60 & 65.58 & 58.12 & 56.99 \\
esp & 72.33 & 36.41 & 61.27 & 65.72 & 73.29 \\
hau & 43.79 & 29.43 & 50.91 & 40.40 & 51.91 \\
hin & 79.73 & 27.59 & 60.59 & 62.19 & 76.91 \\
ibo & 37.40 & 24.31 & 33.18 & 31.90 & 32.85 \\
kin & 31.96 & 19.73 & 34.36 & 26.35 & 32.52 \\
mar & 74.58 & 25.69 & 67.40 & 50.36 & 76.68 \\
% orm & 31.56 & 22.89 & 29.84 & 24.25 & 28.15 \\
pcm & 38.66 & 34.41 & 48.67 & 45.61 & 45.00 \\
ptbr & 51.60 & 25.90 & 45.03 & 41.64 & 51.49 \\
ptmz & 40.44 & 16.70 & 34.06 & 36.52 & 39.58 \\
rus & 73.08 & 29.72 & 62.61 & 61.72 & 76.97 \\
% som & 28.55 & 19.82 & 32.49 & 25.63 & 26.56 \\
sun & 42.67 & 32.20 & 46.33 & 42.10 & 44.61 \\
swa & 27.36 & 17.63 & 29.47 & 26.51 & 33.27 \\
swe & 48.89 & 21.79 & 50.26 & 48.61 & 44.60 \\
tat & 51.58 & 25.12 & 49.84 & 39.44 & 53.86 \\
% tir & 31.13 & 1.46 & 32.93 & 27.16 & 26.49 \\
ukr & 54.76 & 17.16 & 42.34 & 40.15 & 51.19 \\
vmw & 20.41 & 16.03 & 18.96 & 19.00 & 19.09 \\
yor & 24.99 & 16.00 & 23.70 & 19.67 & 27.44 \\
\bottomrule
\end{tabular}
\caption{Average F1-Macro for perceived emotion prediction in Track A per LLM and language.}
\end{table*}

==> tables/track_a_lms.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lccccc}
\toprule
Language & LaBSE & RemBERT & XLM-R & mBERT & mDeBERTa \\
\midrule
afr & 30.76 & 37.14 & 10.82 & 25.87 & 16.66 \\
%amh & 64.39 & 16.95 & 53.67 & 26.91 & 42.71 \\
arq & 45.46 & 41.41 & 31.98 & 41.75 & 29.68 \\
ary & 45.81 & 47.16 & 40.66 & 36.87 & 38.00 \\
chn & 53.47 & 53.08 & 58.48 & 49.61 & 44.47 \\
deu & 55.02 & 64.23 & 55.37 & 46.78 & 44.09 \\
eng & 64.24 & 70.83 & 67.30 & 58.26 & 58.94 \\
esp & 72.88 & 77.44 & 29.85 & 54.41 & 60.17 \\
hau & 58.49 & 59.55 & 36.95 & 47.33 & 48.59 \\
hin & 75.25 & 85.51 & 33.71 & 54.11 & 54.34 \\
ibo & 45.90 & 47.90 & 18.36 & 37.23 & 31.92 \\
kin & 50.64 & 46.29 & 32.93 & 35.61 & 38.00 \\
mar & 80.76 & 82.20 & 78.95 & 60.01 & 66.01 \\
%orm & 36.60 & 42.63 & 20.72 & 26.50 & 29.84 \\
pcm & 51.30 & 55.50 & 52.03 & 48.42 & 46.21 \\
ptbr & 42.60 & 42.57 & 15.40 & 32.05 & 24.08 \\
ptmz & 36.95 & 45.91 & 30.72 & 14.81 & 21.89 \\
ron & 9.10 & 0.00 & 8.73 & 8.73 & 16.68 \\
rus & 75.62 & 83.77 & 78.76 & 61.81 & 54.79 \\
%som & 42.25 & 42.16 & 35.37 & 4.97 & 34.68 \\
sun & 36.93 & 37.31 & 19.66 & 27.88 & 21.65 \\
swa & 27.53 & 22.65 & 22.71 & 22.99 & 22.84 \\
swe & 49.23 & 51.98 & 34.63 & 44.24 & 40.90 \\
tat & 57.71 & 53.94 & 26.48 & 43.49 & 35.02 \\
%tir & 47.02 & 39.10 & 20.13 & 24.88 & 39.46 \\
ukr & 50.07 & 53.45 & 17.77 & 31.74 & 28.55 \\
vmw & 21.13 & 12.14 & 9.92 & 10.28 & 11.13 \\
yor & 32.55 & 9.22 & 11.94 & 21.03 & 17.88 \\
\bottomrule
\end{tabular}
\caption{Average F1-Macro for perceived emotion prediction in Track A per model and language.}
\label{tab:main_results_track_a_lms}
\end{table*}

==> tables/track_b_llms.tex <==
\begin{table*}
\centering
\begin{tabular}{lrrrrr}
\toprule
 & Qwen2.5-72B & Dolly-v2-12B & Llama-3.3-70B & Mixtral-8x7B & DeepSeek-R1-70B \\
\midrule
%amh & 21.15 & -4.32 & 33.93 & 13.22 & 29.08 \\
arq & 29.54 & 3.80 & 36.29 & 31.05 & \textbf{36.37} \\
chn & 46.17 & 8.11 & \textbf{51.86} & 46.52 & 48.57 \\
deu & 43.30 & 7.43 & 53.46 & 47.60 & \textbf{54.78} \\
eng & \textbf{55.99} & 13.35 & 44.14 & 55.26 & 48.08 \\
esp & 51.11 & 10.49 & 51.64 & 55.54 & \textbf{60.74} \\
ptbr & 38.20 & 9.02 & 40.90 & 39.17 & \textbf{46.72} \\
rus & 58.25 & 13.96 & 57.56 & 56.01 & \textbf{62.28} \\
ukr & 37.74 & 6.04 & 36.99 & 38.74 & \textbf{43.54} \\
\bottomrule
\end{tabular}
\caption{Average Pearson correlation for perceived emotion intensity prediction in Track B per LLM and language.}
\end{table*}

==> tables/track_b_lms.tex <==
\begin{table}[ht]
%\small
%\resizebox{\textwidth}{
\centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Lang.} &\textbf{LaBSE} & \textbf{RemBERT} & \textbf{XLM-R} & \textbf{mBERT} & \textbf{mDeBERTa} \\
\midrule
%amh & 44.19 & 48.97 & 41.33 & 42.19 & 11.73 \\
arq & 1.42 & 1.64 & 0.00 & 0.00 & 0.00 \\
chn & 23.37 & 40.53 & 36.92 & 21.96 & 23.25 \\
deu & 28.93 & 56.21 & 38.30 & 17.35 & 18.14 \\
eng & 35.34 & 64.15 & 37.36 & 25.74 & 8.85 \\
esp & 56.89 & 72.59 & 55.72 & 27.94 & 29.18 \\
hau & 26.13 & 27.03 & 24.68 & 2.79 & 0.00 \\
ptbr & 20.62 & 29.74 & 18.24 & 8.36 & 1.32 \\
ron & 35.57 & 55.66 & 37.77 & 21.99 & 4.63 \\
rus & 68.43 & 87.66 & 68.96 & 37.63 & 5.03 \\
ukr & 13.75 & 39.94 & 36.16 & 4.32 & 3.51 \\
\bottomrule
\end{tabular}
}\caption{Average Pearson correlation coefficient for perceived emotion intensity prediction in Track B per model and language.}
\label{tab:main_results_track_b_lms}
\end{table}

==> tables/track_c_lms.tex <==
\begin{table*}
\centering
\begin{tabular}{lccccc}
\toprule
Language & LaBSE & RemBERT & XLM-R & mBERT & mDeBERTa \\
\midrule
\texttt{afr} & 35.12 & 35.04 & 41.66 & 16.95 & 33.25 \\
\texttt{arq} & 35.93 & 33.78 & 35.87 & 31.38 & 35.92 \\
\texttt{ary} & 42.83 & 35.46 & 33.88 & 24.83 & 36.28 \\
\texttt{chn} & 45.28 & 24.56 & 53.84 & 21.61 & 42.41 \\
\texttt{deu} & 42.45 & 46.84 & 47.26 & 28.60 & 42.61 \\
\texttt{eng} & 36.71 & 37.54 & 37.60 & 18.80 & 35.30 \\
\texttt{esp} & 54.56 & 57.37 & 44.52 & 30.09 & 37.09 \\
\texttt{hau} & 38.46 & 31.98 & 16.69 & 15.59 & 32.80 \\
\texttt{hin} & 69.78 & 13.75 & 69.96 & 36.94 & 57.74 \\
\texttt{ind} & 47.50 & 37.64 & 25.39 & 26.87 & 35.68 \\
\texttt{jav} & 46.24 & 46.38 & 20.39 & 26.16 & 35.34 \\
\texttt{ibo} & 18.13 & 7.49 & 10.42 & 9.94 & 9.52 \\
\texttt{kin} & 30.35 & 18.38 & 13.12 & 20.90 & 17.30 \\
\texttt{mar} & 74.65 & 77.24 & 76.21 & 42.32 & 54.05 \\
\texttt{pcm} & 33.29 & 1.01 & 21.08 & 22.55 & 25.39 \\
\texttt{ptbr} & 41.51 & 41.84 & 43.09 & 23.86 & 34.42 \\
\texttt{ptmz} & 31.44 & 29.67 & 7.30 & 13.54 & 24.46 \\
\texttt{ron} & 60.55 & 60.58 & 60.42 & 53.38 & 61.04 \\
\texttt{rus} & 61.32 & 70.43 & 21.14 & 37.15 & 29.70 \\
\texttt{swa} & 21.66 & 18.99 & 16.94 & 18.61 & 14.94 \\
\texttt{swe} & 44.24 & 51.18 & 10.08 & 28.86 & 43.28 \\
\texttt{tat} & 60.66 & 44.54 & 39.58 & 35.81 & 47.72 \\
\texttt{ukr} & 44.37 & 49.56 & 34.06 & 25.69 & 35.12 \\
\texttt{vmw} & 9.65 & 5.22 & 12.66 & 12.11 & 11.74 \\
\texttt{xho} & 31.39 & 12.73 & 11.48 & 17.08 & 22.86 \\
\texttt{yor} & 11.64 & 5.33 & 6.64 & 9.62 & 10.03 \\
\texttt{zul} & 18.16 & 15.26 & 10.92 & 13.04 & 13.87 \\
\bottomrule
\end{tabular}
\caption{Average F1-Macro for perceived emotion prediction in Track C per model and language. We trained on all languages in one language family except the focal language (each row in the table is one focal language) and evaluate on the test set of the focal language.}
\label{tab:main_results_track_c_lms}
\end{table*}

